keV Sterile Neutrino Dark Matter from Singlet Scalar Decays: Basic Concepts and Subtle Features

We perform a detailed and illustrative study of the production of keV sterile neutrino Dark Matter (DM) by decays of singlet scalars in the early Universe. In the current study we focus on providing a clear and general overview of this production mechanism. For the first time we study all regimes possible on the level of momentum distribution functions, which we obtain by solving a system of Boltzmann equations. These quantities contain the full information about the production process, which allows us to not only track the evolution of the DM generation but to also take into account all bounds related to the spectrum, such as constraints from structure formation or from avoiding too much dark radiation. In particular we show that this simple production mechanism can, depending on the regime, lead to strongly non-thermal DM spectra which may even feature more than one peak in the momentum distribution. These cases could have particularly interesting consequences for cosmological structure formation, as their analysis requires more refined tools than the simplistic estimate using the free-streaming horizon. Here we present the mechanism including all concepts and subtleties involved, for now using the assumption that the effective number of relativistic degrees of freedom is constant during DM production, which is applicable in a significant fraction of the parameter space. This allows us to derive analytical results to back up our detailed numerical computations, thus leading to the most comprehensive picture of keV sterile neutrino DM production by singlet scalar decays that exists up to now.

==> JCAP_proofs <==
List of corrections
====================
1) page 4, paragraph 2, line 8 (the line directly after formula 2.1) 	the word "in" before previously is redundant

2) page 4, paragraph 2, line 9 						after the word "details", the word "of" is missing and should be inserted

3) page 5, paragraph 2, line 6 						it should read "if one used" instead of "if one uses"

4) page 5, paragraph 2, line 11						the word "further" should be replaced by "future"

5) page 8, paragraph 2, line 5						it should read "space, as we will illustrate" instead of "space, which we will illustrate"

6) page 9, formula (3.10)						there is a erroneous factor f_S\left(x,r\right) in the nominator, which must be taken out

7) page 9, paragraph 3, line 6 (the line directly after formula 3.14):	in the definition of x_min, there is a prime missing. Please replace 
									$\sub{\hat{x}}{min} = \left\|x-r^2/\left(4x\right)\right\|$ in the source code by
									$\sub{\hat{x}}{min} = \left\|x-{r'}^2/\left(4x\right)\right\|$	

8) page 10, paragraph 1, line 1						it should read "two main cases, the scalar" instead of "two main cases: the scalar"	
9) page 10, paragraph 1, line 3						the line shall read "interacting, thus undergoing freeze-in like a FIMP:" 
									instead of "interacting, thus undergoing freeze-in like a FIMP. These are:" 
	
10) page 5, paragraph 2 of footnote 5, line 10				it should read "of which it is however unclear" instead of "from which it is however unclear"

11) page 13, paragraph 1 of subsection  4.3, line 3			it shall read "and then compare" instead of "and to compare"

11) page 13, formula 4.7		 				the left-hand side should be "\sub{\Omega}{DM} h^2" instead of "\Omega h^2", to be more consistent with the labels in the figures and the
									rest of the text.

12) page 14, paragraph 1 of subsection 5.1, line 2			the text should read "which will make clear" instead of "which will make it clear"

13) page 14, paragraph 1 of subsection 5.1, line 3			no comma after "Moreover"

14) page 14, paragraph 3 of subsection 5.1., line 10			it should read "(d.o.f.) is implemented by" instead of "(d.o.f.) is treated by" 

15) page 15 paragraph 2, line 5						There is a . missing between "account" and "Thereby"

16) page 15, paragraph 2 of subsection 5.2, line 1			it should read "for different values of the" instead of "for different values in the"

17) page 16, paragraph 2, line 2					it should read "while the right one would indicate hot DM in both cases." instead of "while the right one would indicate hot DM."

18) page 18, paragraph 2, line 4					please replace "Taking again the benchmark value $m_S = \unit{1}{TeV}$ and taking" by 
									"Taking again the benchmark value $m_S = \unit{1}{TeV}$ and using"

---------------------------


19) page 22, paragraph 1, line 3					it should read "In figure 8, we again display" instead of "In figure 8, we show again"

20) page 24, paragraph 2 of subsection 6.3, line 2			please replace "kinetic part of their energy density to the energy $\ssscript{\rho}{term}{ferm}$ density of 
									a perfectly relativistic (i.e.~massless) fermionic species" by
									"kinetic part of their energy density to the energy density $\ssscript{\rho}{term}{ferm}$ of 
									a perfectly relativistic (i.e.~massless) fermionic species"

21) page 25, line 5 of footnote 11					it should read "per definition, so that" instead of "per definition so that"

22) page 31, line directly before formula A.11				there should be a : after "reads"

23) page 31, line directly before formula A.12				there should be a : after "reads"

24) page 32, formulae A.17, A.18 and third line after A.18		please replace $\vec{p}'$ by $\vec{p'}$ which would be more readable and also consistent with the notation of A.15

25) page 33, line directly after B.1					please replace the word "numerical" at the end of the line by "fitted"





List of optional changes in the layout
======================================
a) Maybe Figure 5 can be put one page later to be in closer connection to the corresponding text


==> JCAP_proofs_2 <==
Dear Editors,

thank you for sending us the revised version and giving us the chance for some final checks.
We rechecked all formulas in the appendix and found a couple of typos in some intermediary results.
The final results remain untouched.

Here is a list of the complete formulas, as they should read. Please replace the existing versions by the new ones.

(1)	equation (A.12)

\begin{align}
{C}_{SS \rightarrow hh}^{S}\left(q\right) &=  \left(-\frac{1}{2E_q}\right) \int \invps{q'} \invps{p} \invps{p'} \frac{4\lambda^2}{8 \pi} \nonumber \\
 &\times \twopin{4} \deltadistn{4}{q+q'-p-p'}f_S\left(q\right) f_S\left(q'\right) \nonumber \\
&= -\frac{f_S\left(q\right)}{2E_q}\frac{4\lambda^2}{16 \pi} \int \invps{q'} f_S\left(q'\right) \sqrt{\frac{\left(E_q +E_{q'}\right)^2 -qq'\cos \theta - 4m_h^2}{\left(E_q +E_{q'}\right)^2 -qq'\cos \theta}} \,.
\label{eq:BoltzmannScalarAnn}
\end{align}



(2)	equation (A.15)

\begin{align}
 C_{S\rightarrow NN}^{S}\left(q\right) &= - \frac{1}{2 E_q} \iint \frac{2\diffd ^3 p}{\left(2\pi\right)^3 2 E_{p}}  \frac{2\diffd ^3 p'}{\left(2\pi\right)^3 2 E_{p'}} \frac{1}{2} y^2 E_p E_{p'} \left[1 - \frac{\vec{p} \cdot \vec{p'}}{E_p E_{p'}}\right] \twopin{4} \deltadistn{4}{q -p -p'} f_s\left(q\right)\nonumber \\
&= - f_S\left(q\right) \Gamma \frac{m_S}{E_q} \, ,
\label{eq:CollisionTermS:SToNNDerivation}
\end{align}



(3)	equation (A.17)

\begin{align}
C_{S\rightarrow NN}^{N} = 2\times \frac{1}{2E_p} \iint  \frac{2\diffd ^3 p'}{\left(2\pi\right)^3 2 E_{p'}} \invps{p_S} \twopin{4} \deltadist{E_{p_S} - E_p -E_{p'}} \deltadistn{3}{\vec{p}_S -\vec{p} -\vec{p'}} 2 \Msquared f_S\left(p_S,t \right) \,,
 \label{eq:CSNNN}
\end{align}


---------------------------
These are now the final proofs. We apologize for the inconvenience.

Best regards,
Alexander Merle & Maximilian Totzauer

